Bayesian Exploration with Heterogeneous Agents

It is common in recommendation systems that users both consume and produce information as they make strategic choices under uncertainty. While a social planner would balance "exploration" and "exploitation" using a multi-armed bandit algorithm, users' incentives may tilt this balance in favor of exploitation. We consider Bayesian Exploration: a simple model in which the recommendation system (the "principal") controls the information flow to the users (the "agents") and strives to incentivize exploration via information asymmetry. A single round of this model is a version of a well-known "Bayesian Persuasion game" from [Kamenica and Gentzkow]. We allow heterogeneous users, relaxing a major assumption from prior work that users have the same preferences from one time step to another. The goal is now to learn the best personalized recommendations. One particular challenge is that it may be impossible to incentivize some of the user types to take some of the actions, no matter what the principal does or how much time she has. We consider several versions of the model, depending on whether and when the user types are reported to the principal, and design a near-optimal "recommendation policy" for each version. We also investigate how the model choice and the diversity of user types impact the set of actions that can possibly be "explored" by each type.

==> private_type_c_old.tex <==
%!TEX root = main.tex

\section{Bayesian Exploration with Reported Types}
\label{sec:private_c}
In this section, we show a BIC scheme for private types when communication is allowed. The main idea is to guess the type of each agent and then use the scheme in Section \ref{sec:public}. In each round, we also ask the agent to report its type in the end. Since this report has nothing to do with the recommended actions received, the agent has no incentive to misreport its type. Our scheme only uses information collected in rounds when the guessed type equals to the actual type and therefore the expected length of each epoch becomes longer than the one in Section \ref{sec:public} (as shown in Lemma \ref{lem:epoch_private}. Once the scheme explores all the explorable type-action pairs, it just shows agents the best action for each type among all explorable actions. 

Algorithm \ref{alg:private_main} is the main procedure of the scheme. It is very similar to the main procedure in Section \ref{sec:public} (Algorithm \ref{alg:public_main}). The only difference is that the scheme guesses types and only uses information collected in rounds when the scheme guesses the type correctly. 

 \begin{algorithm}[H]
    \caption{Main procedure for private types }
    	\label{alg:private_main}
    \begin{algorithmic}[1]
    	\STATE Initial signal $S_1 = \S_1 = \perp$.
	\STATE Initial epoch count $l = 1$. 
	\FOR {$t=1$ to $T$}
		\STATE The principal receives information $I_t$ about $\theta_t$. 
		\STATE Sample $\hat{\theta}_t$ from $\varTheta$ uniformly. Run subroutine Private-Sub-$\hat{\theta}_t$.
		\IF {every type has finished a complete phase in the current epoch}
			\STATE Start a new epoch:
			\STATE $l \leftarrow l + 1$.
			\STATE Let $S_l$ be the type-action-reward triples in rounds when $\bar{\theta}_{\tau} = \hat{\theta}_{\tau}$, and $\S_l$ be the signal structure.
		\ENDIF
	\ENDFOR
     \end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:private_sub} describes the thread when the algorithm guesses the type to be $\theta$. It is very similar to Algorithm \ref{alg:public_sub} in Section \ref{sec:public}. We use the same $L_{\theta}$ as Section \ref{sec:public}.

 \begin{algorithm}[H]
    \caption{Subroutine for type $\theta$: Private-Sub-$\theta$ }
    	\label{alg:private_sub}
    \begin{algorithmic}[1]
	\FOR {each call from Algorithm \ref{alg:public_main}}
		\IF {previous phase has finished ($i_{\theta} > L_{\theta}$) or this is the first call}
			\STATE Start a new phase:
			\IF {$l \leq |\A| \cdot |\varTheta|$}
				\STATE Use the current $S_l$ and $\S_l$ to compute a list of $L_{\theta}$ actions $\alpha_{\theta} \leftarrow $ MaxExplore($\theta, S_l, \S_l$).
			\ELSE
				\STATE Add $L_{\theta}$ copies of the best explored action of type $\theta$ according to signal $S$ into action list $\alpha_{\theta}$. 
			\ENDIF
			\STATE Intialize the index of current phase $i_{\theta} \leftarrow 1$.
		\ENDIF
		\STATE Recommend $(\alpha_{\theta} [i_{\theta}]$ for type $\theta$ and for other types, recommend the best actions given the agents' prior and the fact that $(\alpha_{\theta} [i_{\theta}]$ is recommended for type $\theta$ .
		\STATE Agent reports its type $\bar{\theta}$.
		\IF {$\bar{\theta} = \theta$}
			\STATE $i_{\theta} \leftarrow i_{\theta} + 1$.
		\ENDIF
	\ENDFOR
     \end{algorithmic}
\end{algorithm}

For similar reasons as Claim \ref{clm:public_BIC}, we have the following claim. 
\begin{claim}
\label{clm:private_BIC}
The scheme in this section is BIC. 
\end{claim}

Finally, we prove the main theorem of this section (Theorem \ref{thm:private}). It is based on Lemma \ref{lem:epoch_private} and Lemma \ref{lem:exp_private}.

\begin{lemma}
\label{lem:epoch_private}
For any $l>0$, the expected number of rounds of the first $l$ epochs is at most $l \cdot \sum_{\theta\in\varTheta} \frac{2\cdot L_{\theta}\cdot |\varTheta|}{\Pr[\theta]}$. 
\end{lemma}

\begin{proof}
First of all, if a type $\theta$ is guessed correctly $2L_{\theta}$ times, type $\theta$ must have finished a complete phase in these rounds. Therefore, the expected number of rounds of an epoch is at most the expected number of rounds in which each type $\theta$ is guessed correctly at least $2L_{\theta}$ times. The latter expectation can be easily bounded by $\sum_{\theta\in\varTheta} \frac{2L_{\theta}\cdot |\varTheta| }{\Pr[\theta]}$. Therefore, the expected number of rounds of the first $l$ epochs is at most $l \cdot \sum_{\theta\in\varTheta} \frac{2L_{\theta}\cdot |\varTheta|}{\Pr[\theta]}$. 
\end{proof}

\begin{lemma}
\label{lem:exp_private}
For each state $\omega$, Algorithm \ref{alg:private_main} explores all the eventually explorable actions (i.e. $\A_{\omega,\theta}^{exp}$) for each type $\theta$ by the end of $|\A|\cdot |\varTheta|$ epochs. 
\end{lemma}

\begin{proof}
Fix state $\omega$. Consider any type sequence $\theta_1, \theta_2, ..., \theta_T$ that are the types encountered by Algorithm \ref{alg:private_main} in each round. And consider another type sequence $\bar{\theta}_1,\bar{\theta}_2, ...,\bar{\theta}_T$ that are the guesses by Algorithm \ref{alg:private_main}. Assume Algorithm \ref{alg:private_main} finished the $(|\A|\cdot |\varTheta|)$-th epoch after round $t$. Let $r_1<r_2 < \cdots < r_{\tau} = t$ be the rounds that Algorithm \ref{alg:private_main} guesses the type correctly (i.e. $\theta = \bar{\theta}$) in the first $t$ rounds. Assume Algorithm \ref{alg:private_main} uses randomness $R$ for MaxExplore. Now consider Algorithm \ref{alg:public_main} also uses the same randomness $R$ for MaxExplore when facing types $\theta_{r_1},\theta_{r_2},...,\theta_{r_{\tau}}$ in each round. By the definition of Algorithm \ref{alg:private_main} and Algorithm \ref{alg:public_main}, it's not hard to check that the $i$-th round of Algorithm \ref{alg:public_main} and the $r_i$-th round of Algorithm \ref{alg:private_main} play the same action. 

Since Algorithm \ref{alg:private_main} finishes $|\A|\cdot |\varTheta|$ epochs at round $t$, Algorithm \ref{alg:public_main} also finishes $|\A|\cdot |\varTheta|$ epochs at round $\tau$. By Lemma \ref{lem:exp_public}, we know Algorithm \ref{alg:public_main} has explored all the eventually explorable actions by the end of round $\tau$. Therefore,  Algorithm \ref{alg:private_main} has explored all the eventually explorable actions by the end of round $t$ (i.e. the end of $|\A|\cdot |\varTheta|$ epochs).
\end{proof}

\begin{theorem}
\label{thm:private}
We have a BIC recommendation policy of $T$ rounds with expected total reward at least $\left(T - C \right) \cdot \OPT$ for some constant $C = |\A| \cdot |\varTheta| \cdot \sum_{\theta\in\varTheta} \frac{2L_{\theta}\cdot |\varTheta|}{\Pr[\theta]}$. 
\end{theorem}

\begin{proof}
First of all, by Claim \ref{clm:private_BIC}, Algorithm \ref{alg:private_main} is BIC. 

By Lemma \ref{lem:exp_private}, for each state $\omega$, Algorithm \ref{alg:private_main} explores all the eventually explorable actions (i.e. $\A_{\omega,\theta}^{exp}$) for each type $\theta$ by the end of $|\A|\cdot |\varTheta|$ epochs. After that, for each type $\theta$, Algorithm \ref{alg:private_main} will always recommend action $ \max_{a \in \A_{\omega,\theta}^{exp}} u(\theta, a, \omega)$. Therefore Algorithm \ref{alg:private_main} gets reward $OPT$ except rounds in first $|\A|\cdot |\varTheta|$ epochs. By Lemma \ref{lem:epoch_private}, we know that the expected number of rounds of the first  $|\A|\cdot |\varTheta|$ epochs is at most $C$. Therefore, Algorithm \ref{alg:private_main} has expected total reward at least  $\left(T - C \right) \cdot \OPT$.

\end{proof}

==> private_type_nc_temp.tex <==
%!TEX root = main.tex

\section{Bayesian Exploration with Private Types and No Communication (Approach 1)}



\subsection{Exporability and Benchmark}

\begin{definition}
A menu $m: \varTheta \rightarrow \A$ is a mapping from the type space $\varTheta$ to the action space $\A$. We use $\M$ to denote the set of all menus.
\end{definition}

\begin{claim}
Each single round of a BIC scheme can be considered as a distribution of menus.
\end{claim}

\begin{definition}
A menu $m$ is eventually-explorable, for a given state $\omega$, if there exists a BIC recommendation policy $\pi$ and some round $t$ such that $\Pr[\pi^t= m]> 0$. The set of all such menus is denoted as $\M_{\omega}^{exp}$.
\end{definition}

\begin{definition}[Benchmark]
Define benchmark as 
\[
\OPT = \sum_{\theta \in \varTheta, \omega\in \varOmega} \Pr[\omega] \cdot \Pr[\theta] \cdot \max_{m \in \M_{\omega}^{exp}} u(\theta, m(\theta), \omega).
\]
\end{definition}

\begin{claim}
Any $\delta$-BIC recommendation policy of $T$ rounds has expected total reward at most $T \cdot\OPT$.  
\end{claim}

\begin{theorem}
\label{thm:private_nocc}
We have a BIC recommendation policy of $T$ rounds with expected total reward at least $\left(T - C \right) \cdot \OPT$. 
\end{theorem}

\subsection{BIC Exploration Scheme with Sample Distributions}
In this subsection, we consider a simpler case in which the description of the distribution of samples of a menu is directly given to the scheme. Samples of a menu is defined as following: 
\begin{definition}[Samples of a Menu]
Given a menu $m$ and an agent's type $\theta$ sampled from the type distribution, an action-reward pair will be deteremined assuming the agent is following the menu. Such action-reward pair is called a sample of the menu $m$. 
\end{definition}
Notice that the description of the distribution of samples of a menu $m$ is a deterministic function of $m$ and state $\omega$. 

In this simpler setting, we can also define eventually-explorable menus and the benchmark. To distiguish this simpler setting with the original setting, we put a $\Ds$ in the notations:

\begin{definition}
A menu $m$ is eventually-explorable in the simpler setting, for a given state $\omega$, if there exists a BIC recommendation policy $\pi$ in the simpler setting and some round $t$ such that $\Pr[\pi^t= m]> 0$. The set of all such menus is denoted as $\Ds\M_{\omega}^{exp}$.
\end{definition}

\begin{definition}[Benchmark]
Define benchmark in the simpler setting as 
\[
\Ds\OPT = \sum_{\theta \in \varTheta, \omega\in \varOmega} \Pr[\omega] \cdot \Pr[\theta] \cdot \max_{m \in \Ds\M_{\omega}^{exp}} u(\theta, m(\theta), \omega).
\]
\end{definition}

To connect the simpler setting with the original setting, we use the following claim to show that simpler setting is easier in terms of exploration and has a no smaller benchmark.
\begin{claim}
$\Ds OPT \geq OPT$ and for all $\omega$, $\M_{\omega}^{exp} \subseteq \Ds\M_{\omega}^{exp}$. 
\end{claim}

\begin{theorem}
\label{thm:private_noccd}
We have a BIC recommendation policy in the simpler setting of $T$ rounds with expected total reward at least $\left(T - C \right) \cdot \OPT$. 
\end{theorem}



==> public_type_old.tex <==
%!TEX root = main.tex

\section{Bayesian Exploration with Public Types}
\label{sec:public}
In this section, we show a BIC scheme for public types (as in Theorem \ref{thm:public}). We formally state Theorem \ref{thm:public} in Section \ref{sec:public_bench} and we prove it in Section \ref{sec:public_single} and \ref{sec:public_main}.

\subsection{Explorability and Benchmark}
\label{sec:public_bench}
In this subsection, we define the benchmark and state our main theorem (Theorem \ref{thm:public}).

\begin{definition}
\label{def:public_exp}
An action $a$ of type $\theta$ is eventually-explorable, for a given state $\omega$, if there exists a BIC recommendation policy $\pi$ and some round $t$ such that $\Pr[\pi^t(\theta)= a]> 0$. The set of all such actions for state $\omega$ and type $\theta$ is denoted as $\A_{\omega,\theta}^{exp}$.
\end{definition}

\begin{definition}[Benchmark]
Define benchmark as
\[
\OPT = \sum_{\theta \in \varTheta, \omega\in \varOmega} \Pr[\omega] \cdot \Pr[\theta] \cdot \max_{a \in \A_{\omega,\theta}^{exp}} u(\theta, a, \omega).
\]
\end{definition}

Notice that for a given state $\omega$ and type $\theta$, any BIC recommendation policy can only recommend an action in $\A_{\omega,\theta}^{exp}$. We can simply get the following claim which says that no BIC recommendation policy can get expected per round reward better than the benchmark:
\begin{claim}
Any BIC recommendation policy of $T$ rounds has expected total reward at most $T \cdot\OPT$.
\end{claim}

On the other hand, we construct a BIC recommendation policy that nearly achieves the benchmark. It's proved in the following subsections.
\begin{theorem}
\label{thm:public}
We have a BIC recommendation policy of $T$ rounds with expected total reward at least $\left(T - C \right) \cdot \OPT$ for some constant $C$ which does not depend on $T$.
\end{theorem}

\subsection{Single-round Exploration}
\label{sec:public_single}
%This section is very similar to the EC16's paper, we include this section to make our paper self-contained.

In this subsection, we consider a single round of the Bayesian exploration. As we only consider one round, we fix the agent's type in this round to be $\theta$. 

In a single round, the principal receives a random variable $S$ (we call it a signal) which is a function of the history of previous rounds and randomness of the recommendation policy. This function is determined before all rounds start and is known to the principal and all agents. In this single round, the principal computes a (randomized) mapping from the signal to a suggested action. We specify the signal structure $\S$ of signal $S$ by the signal support $\X$ and a joint distribution on $(\X, \varOmega)$.  


\begin{definition}
Consider a single-round of Bayesian exploration when the principal receives signal $S$ with signal structure $\S$. An action $a \in \A$ is called signal-explorable, for a given realized signal $s$, if there exists a single-round BIC recommendation policy $\pi$ such that $\Pr[\pi(s) = a] > 0$. The set of all such actions is denoted as $\EX_s[\S]$. The signal-explorable set is defined as $\EX[\S] = \EX_S[\S]$.
\end{definition}

Note that $\EX_s[\S]$ is a fixed subset and $\EX[\S]$ is a random variable whose realization is determined by the realization of signal $S$.

\subsubsection{Information Monotonicity}
In the following definition, we define a way to compare two signals. Intuitively, the condition $I(S';\Omega|S)= 0$  means if one is given random variable $S$, one can learn no information from $S'$ about $\Omega$. In this case, we show in Lemma \ref{lem:infomono} that the signal-explorable set of $S'$ is contained the signal-explorable set of $S$.
\begin{definition}
Let $S$ and $S'$ be two random variables and $\S$ and $\S'$ be their signal structures. We say random variable $S$ is at least as informative as random variable $S'$ about state $\Omega$ if $I(S' ; \Omega|S) = 0$. Notice $I(S';\Omega|S)$ does not only depend on the signal structures $\S$ and $\S'$. It can also depend on the joint distribution between $S$ and $S'$.
\end{definition}

\begin{lemma}
\label{lem:infomono}
Let $S$ and $S'$ be two random variables and $\S$ and $\S'$ be their signal structures. If $S$ is at least as informative as $S'$ about state $\Omega$ (i.e. $I(S' ; \Omega|S) = 0$), then $\EX_{s'}[\S'] \subseteq \EX_s[\S]$ for all $s' ,s$ such that $\Pr[S= s, S'= s'] > 0$.
\end{lemma}

\begin{proof}
Consider any BIC recommendation policy $\pi'$ for signal structure $\S'$. We construct $\pi$ for signature structure $\S$ by setting $\Pr[\pi(s) = a] = \sum_{s'} \Pr[\pi'(s') = a] \cdot Pr[S' = s'|S = s]$. It's easy to check $\pi$ is BIC. For any $s', s ,a$ such that $Pr[S' = s',S = s] >0 $ and $\Pr[\pi'(s') = a] >0$, we have $\Pr[\pi(s) = a] > 0$. This implies $\EX_{s'}[\S'] \subseteq \EX_s[\S]$.
\end{proof}

\subsubsection{Max-Support Policy}
For a given realized signal $s \in \X$ and an action $a \in \A$, we solve the following LP to check if $a$ is signal-exlporable given realized signal $s$. The LP is parameterized by the signal structure $\S$ together with the realized signal $s$. 

\begin{figure}[H]
\begin{mdframed}
\begin{alignat*}{2}
  \textbf{maximize }   & x_{a,s}\  \\
  \textbf{subject to: } & \sum_{\omega \in \varOmega, s' \in \X} \Pr[\omega] \cdot \Pr[s' | \omega] \cdot \left(u(\theta, a', \omega) - u(\theta, a'', \omega)\right) \cdot x_{a',s'} \geq 0   &\ & \forall a',a'' \in \A \\
                       & \sum_{a'\in \A} x_{a',s'} = 1,  \ &\ & \forall s' \in \X \\
                       & x_{a',s'} \geq 0,  \ &\ & \forall s' \in \X, a'\in \A \\
\end{alignat*}
\end{mdframed}
%\caption{LP}
\label{fig:public_lp}
\end{figure}

Notice that the constraints in the above LP characterize any BIC recommendation policy. Therefore we get the following claims.
\begin{claim}
For a given signal $s \in \X$, an action $a \in \A$ is signal-explorable if and only if the above LP has a positive solution. 
\end{claim}

\begin{claim}
When the LP has a positive solution, define $\pi^{a,s}$ as $\Pr[\pi^{a,s}(s') = a'] = x_{a',s', } \forall a' \in \A, s' \in \X$. Then $\pi^{a,s}$ is a single-round BIC recommendation policy such that $\Pr[\pi^{a,s}(s) = a] > 0$
\end{claim}

\begin{definition}[Max-support policy]
Given a signal structure $\S$, a BIC recommendation policy $\pi$ is called the max-support policy if $\forall s \in \X$  and signal-explorable action $a\in \A$ given $s$, $\Pr[\pi(s) = a] > 0$.
\end{definition}


We can get a max-support policy $\pi^{max}$ by averaging over BIC recommendation policies for signal explorable actions.
\begin{claim}
\label{clm:pimax}
The following $\pi^{max}$ is a BIC and max-support policy. 
\[
\pi^{max} = \frac{1}{|\X|} \sum_{s \in \X} \frac{1}{|\EX_s[\S]|} \sum_{a \in \EX_s[S]} \pi^{a,s}.
\]
\end{claim}

\subsubsection{MaxExplore}
\label{sec:public_maxe}
%This section is very similar to the EC16's paper, we include this section to make our paper self-contained.

In this subsubsection, we show a subroutine MaxExplore which converts $\pi^{max}$ into a sequence of actions. We are going to assume $L_{\theta} \geq \max_{a,s: \Pr[\pi^{max}(s)=a] \neq 0} \frac{1}{\Pr[\pi^{max}(s)=a]}$.

The goal of this subroutine MaxExplore is to make sure that for any signal-explorable action $a$ (i.e. $\Pr[\pi^{max}(s) = a] > 0$), $a$ shows up at least once in the sequence with probability exactly 1. On the other hand, we want that the action of each specific location in the sequence has marginal distribution same as $\pi^{max}$. 

To achieve this goal, the first idea would be to put $C_a = L_{\theta} \cdot \Pr[\pi^{max}(S) = a]$ copies of action $a$ into a sequence of length $L_{\theta}$ and randomly permute the sequence. However, the problems are that $C_a$ might not be an integer and $C_a$ can be smaller than 1. We solve the later problem by picking $L_{\theta}$ large enough such that $C_a \geq 1$ for all $a$ satisfying $\Pr[\pi^{max}(S) =a] > 0$. We solve the former problem by first putting $\lfloor C_a \rfloor$ copies of action $a$ into the sequence and then sampling the rest ($L_\theta - \sum_a \lfloor C_a \rfloor$ actions) according to $\pi^{max}$. For details, see the following pseudo-code (Algorithm \ref{alg:public_explore}). 
 \begin{algorithm}[H]
    \caption{Subroutine MaxExplore}
    	\label{alg:public_explore}
    \begin{algorithmic}[1]
	\STATE \textbf{Input:} type $\theta$, signal $S$ and signal structure $\S$.
	\STATE \textbf{Output:} a list of actions $\alpha$
	\STATE Compute $\pi^{max}$ as stated in Claim \ref{clm:pimax}.
	%\IF {$l \leq |\A| \cdot |\varTheta|$}
		\STATE Initialize $Res = L_{\theta}$.
		\FOR {each action $ a \in \A$}
							\STATE $C_a \leftarrow  L_{\theta} \cdot \Pr[\pi^{max}(S) = a]$
                     		\STATE Add $\lfloor C_a \rfloor$ copies of action $a$ into list $\alpha$.
			\STATE $Res \leftarrow Res -\lfloor C_a \rfloor $.
			\STATE $p^{Res}(a)\leftarrow  C_a -  \lfloor C_a\rfloor$
		\ENDFOR
		\STATE $p^{Res}(a) \leftarrow p^{Res}(a) / Res$, $\forall a \in \A$.
		\STATE Sample $Res$ many actions from distribution according to $p^{Res}$ independently and add these actions into $\alpha$.
		\STATE Randomly permute the actions in $\alpha$.
	%\ELSE
		%\STATE Add $L_{\theta}$ copies of the best explored action of type $\theta$ according to signal $S$ into action list $\alpha$.
	%\ENDIF
	\RETURN $\alpha$.	
     \end{algorithmic}
\end{algorithm}

Such conversion is exactly the same as \cite{ICexplorationGames-ec16-working}, we have the following two claims.

\begin{claim}
\label{clm:maxexplore}
Given type $\theta$ and signal $S$, MaxExplore explores all the signal-explorable actions.
\end{claim}

\begin{claim}
MaxExplore runs in time polynomial in $L_{\theta}$, $|\A|$, $|\varOmega|$ and $|\X|$ (size of the support of the signal). 
\end{claim}

\subsection{Main Scheme}
\label{sec:public_main}
In this subsection, we show our main scheme which explores all the eventually-explorable actions and then advises the agents to choose the best actions among eventually-explorable actions.

Algorithm \ref{alg:public_main} is the main procedure of our recommendation policy . For each type $\theta$, the algorithm activates a separate thread (Sub-$\theta$) whenever type $\theta$ shows up in a round and deactivates the thread after that round. 

Algorithm \ref{alg:public_main} proceeds in phases. We have two types of phases: global phases and local phases. Each round $t$ will be placed in exactly one global phase and also one local phase of its type $\theta_t$. Global phases are applied to all $T$ rounds and these rounds are partitioned into global phases of consecutive rounds. Local phases for type $\theta$ are only applied to rounds in which the agent's type is $\theta$. These rounds are sorted according to their global orders and are partitioned into local phases of $L_\theta$ consecutive rounds in that ordering. We pick $L_{\theta}$ to be at least $\max_{a,s: \Pr[\pi(s)=a] \neq 0} \frac{1}{\Pr[\pi(s)=a]}$ for all $\pi$ that might be chosen as $\pi^{max}$ in Algorithm \ref{alg:public_main} such that $L_{\theta}$ satisfies the guarantee required in Section \ref{sec:public_maxe}.

The partition of global phases depends on the partitions of local phases. In particular, Algorithm \ref{alg:public_main} starts a new global phase when all the types have complete local phases in the current global phase (here ``complete'' means the local phase both starts and ends in the current global phase). 
 \begin{algorithm}[H]
    \caption{Main procedure for public types }
    	\label{alg:public_main}
    \begin{algorithmic}[1]
    	\STATE Initial signal $S_1 = \S_1 = \perp$.
	\STATE Initial global phase count $l = 1$.
	\FOR {$t=1$ to $T$}
		\STATE Let $\theta_t$ to be the agent type of current round $t$. Run subroutine Sub-$\theta_t$.
		\IF {every type has finished a complete local phase in the current global phase}
			\STATE Start a new global phase:
			\STATE $l \leftarrow l + 1$.
			\STATE Let $S_l$ be the set of type-action-reward triples and $\S_l$ be the signal structure when fixing $\theta_1,...,\theta_t$.
		\ENDIF
	\ENDFOR
     \end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:public_sub} describes the thread for type $\theta$. It is activated whenever the agent in the current round has type $\theta$. It partitions the rounds of type $\theta$ into local phases of fixed length ($L_{\theta}$). Each local phase only uses the information collected before the current global phase starts.

 \begin{algorithm}[H]
    \caption{Subroutine for type $\theta$: Sub-$\theta$ }
    	\label{alg:public_sub}
    \begin{algorithmic}[1]
	\FOR {each call from Algorithm \ref{alg:public_main}}
		\IF {previous local phase has finished ($i_{\theta} > L_{\theta}$) or this is the first call}
			\STATE Start a new local phase:
			\IF {$l \leq |\A| \cdot |\varTheta|$}
				\STATE Use the current $S_l$ and $\S_l$ to compute a list of $L_{\theta}$ actions $\alpha_{\theta} \leftarrow $ MaxExplore($\theta, S_l, \S_l$).
			\ELSE
				\STATE Add $L_{\theta}$ copies of the best explored action of type $\theta$ according to signal $S$ into action list $\alpha_{\theta}$.
			\ENDIF
			\STATE Initialize the index of current local phase $i_{\theta} \leftarrow 1$.
		\ENDIF
		\STATE Suggest action $\alpha_{\theta} [i_{\theta}]$ to the agent.
		\STATE $i_{\theta} \leftarrow i_{\theta} + 1$.
	\ENDFOR
     \end{algorithmic}
\end{algorithm}


The proof plan is to first give an upper bound on the expected number of rounds of a global phase in Lemma \ref{lem:epoch} and then show in Lemma \ref{lem:exp_public} that Algorithm \ref{alg:public_main} explores all the explorable type-action pairs in $|\A| \cdot |\varTheta|$ global phases. We use these two lemmas to prove our main theorem (Theorem \ref{thm:public}) in Corollary \ref{cor:public}.

First of all, it's easy to check that for each agent, it is Bayesian incentive compatible to follow the recommended action if previous agents all follow the recommended actions. Therefore we have the following claim.
\begin{claim}
\label{clm:public_BIC}
Our recommendation policy in this section is BIC.
\end{claim}

\begin{lemma}
\label{lem:epoch}
For any $l>0$, the expected number of rounds of the first $l$ global phases is at most $l \cdot \sum_{\theta\in\varTheta} \frac{2L_{\theta}}{\Pr[\theta]}$.
\end{lemma}

\begin{proof}
First of all, if a type $\theta$ shows up $2L_{\theta}$ times in a global phase, type $\theta$ must have finished a complete global phase in these rounds. Notice that $L_{\theta}$ times might not be enough to guarantee a local phase both starts and ends in the global phase because some local phase can start in one global phase and continue in the next global phase. 

Therefore, the expected number of rounds of a global phase is at most the expected number of rounds in which each type $\theta$ has shown up at least $2L_{\theta}$ times. The latter expectation can be easily bounded by $\sum_{\theta\in\varTheta} \frac{2L_{\theta}}{\Pr[\theta]}$. Therefore, the expected number of rounds of the first $l$ global phase is at most $l \cdot \sum_{\theta\in\varTheta} \frac{2L_{\theta}}{\Pr[\theta]}$.
\end{proof}

Notice that in Algorithm \ref{alg:public_main} the partitions of global phases and local phases depend only on realized types $\theta_1,...,\theta_T$ as each local phase has a fixed length $L_{\theta}$. We then have the following claim.
\begin{claim}
Given $\theta_1,...,\theta_T$ as the realized types in $T$ rounds, the partitions of global phases and local phases in Algorithm \ref{alg:public_main} are fixed.
\end{claim}

\begin{lemma}
\label{lem:exp_public}
For any $l>0$ and a fixed sequence of types $\theta_1,...,\theta_T$ as the types encountered by Algorithm \ref{alg:public_main}, assume Algorithm \ref{alg:public_main} has at least $\min(l, |\A|\cdot |\varTheta|)$ global phases.
For a given state $\omega$, if an action $a$ of type $\theta$ can be explored by a BIC recommendation policy $\pi$ at round $l$ (i.e. $ \Pr[\pi^l(\theta)= a]> 0$), then such action is guaranteed to be explored by Algorithm \ref{alg:public_main} by the end of global phase $\min(l, |\A|\cdot |\varTheta|)$.
\end{lemma}

\begin{proof}
We prove this by induction on $l$ for $l \leq |\A|\cdot |\varTheta|$. Base case $l=1$ is trivial by Claim \ref{clm:maxexplore}. Assuming the lemma is correct for $l-1$, let's prove it's correct for $l$.

Let $S$ be the history of Algorithm \ref{alg:public_main} by the end of global phase $l-1$. By the definition of Algorithm 2, $S = S_{l-1} | \theta_1,...,\theta_T$.  Let $S'$ be the history of $\pi$ in the first $l-1$ rounds. More precisely, $S' = R, H_1,...,H_{l-1}$. Here $R$ is the internal randomness of policy $\pi$ and $H_t = (\Theta_t, A_t, u(\Theta_t, A_t, \Omega))$ is the triple of type, action and reward in round $t$ of policy $\pi$.

First of all, we have
\[
I(S'; \Omega| S) = I(R,H_1,...,H_{l-1}; \Omega| S)  = I(R; \Omega| S) + I(H_1,...,H_{l-1}; \Omega|S, R) = I(H_1,...,H_{l-1}; \Omega|S, R).
\]

By the chain rule of mutual information, we have
\[
 I(H_1,...,H_{l-1}; \Omega|S, R) = I(H_1;\Omega|S,R) + I(H_2;\Omega|S, R ,H_1) + \cdots + I(H_{l-1}; \Omega|S,R,H_1,...,H_{l-2}).
\]

For all $t \in [l-1]$, we have
\begin{align*}
&I(H_t; \Omega|S,R,H_1,...,H_{t-1}) \\
=& I(\Theta_t, A_t, u(\Theta_t, A_t, \Omega); \Omega|S,R,H_1,...,H_{t-1}) \\
=& I(\Theta_t ; \Omega|S,R,H_1,...,H_{t-1}) +  I(A_t, u(\Theta_t, A_t, \Omega); \Omega|S,R,H_1,...,H_{t-1},\Theta_t) \\
=& I(A_t, u(\Theta_t, A_t, \Omega); \Omega|S,R,H_1,...,H_{t-1},\Theta_t). \\
\end{align*}
Notice that the suggested action $A_t$ is a deterministic function of randomness of the recommendation policy $R$,  history of previous rounds $H_1,...,H_{t-1}$ and type in the current round $\Theta_t$. Also notice that, by induction hypothesis, $u(\Theta_t, A_t, \Omega)$ is a deterministic function of $|S,R,H_1,...,H_{t-1},\Theta_t, A_t$. Therefore we have
\[
I(H_t; \Omega|S,R,H_1,...,H_{t-1}) = 0, \forall t \in [l-1].
\]
Then we get
\[
I(S'; \Omega | S) = 0.
\]

By Lemma \ref{lem:infomono}, we know that $\EX[\S'] \subseteq \EX[\S]$. For state $\omega$, there exists a signal $s'$ such that $\Pr[S'=s'|\Omega =\omega] >0 $ and $a \in \EX_{s'} [\S']$. Now let $s$ be the realized value of $S$ given $\Omega = \omega$, we know that $\Pr[S'=s'|S=s] >0$, so $a \in \EX_s[\S]$. By Claim \ref{clm:maxexplore}, we know that a complete local phase of type $\theta$ in global phase $l$ of Algorithm \ref{alg:public_main} will choose action $a$ at least once.

Now we consider the case when $l > |\A| \cdot |\varTheta|$. Define Algorithm $E$ to be the variant of Algorithm \ref{alg:public_main} in the sense that Algorithm $E$ always tries to run MaxExplore (i.e. in Sub-$\theta$, ignores if-condition in step 5 and always runs MaxExplore ). For $l > |\A| \cdot |\varTheta|$, the above induction proof still work on Algorithm $E$. Now notice if in some global phase, no unexplored type-action pair is played, Algorithm $E$'s signal in global phases won't change and after that Algorithm $E$ won't explore any unexplored type-action pair. As there are $ |\A| \cdot |\varTheta|$ type-action pairs, Algorithm $E$ only explores unexplored type-action pair in the first $ |\A| \cdot |\varTheta|$ global phases. Therefore, the first $\min(l,|\A|\cdot |\varTheta|)$ global phases of Algorithm \ref{alg:public_main} explores the same set of type-action pair as the first $l$ global phase of Algorithm $E$.
\end{proof}

\begin{corollary}[Restatement of Theorem \ref{thm:public}]
\label{cor:public}
We have a BIC recommendation policy (Algorithm \ref{alg:public_main}) of $T$ rounds with expected total reward at least $\left(T - C \right) \cdot \OPT$ for constant $C = |\A| \cdot |\varTheta| \cdot \sum_{\theta\in\varTheta} \frac{2L_{\theta}}{\Pr[\theta]}$.
\end{corollary}

\begin{proof}
First of all, by Claim \ref{clm:public_BIC}, Algorithm \ref{alg:public_main} is BIC.

By Lemma \ref{lem:exp_public}, for each state $\omega$, Algorithm \ref{alg:public_main} explores all the eventually explorable actions (i.e. $\A_{\omega,\theta}^{exp}$) for each type $\theta$ by the end of $|\A|\cdot |\varTheta|$ global phases. After that, for each type $\theta$, Algorithm \ref{alg:public_main} will always recommend action $ \arg\max_{a \in \A_{\omega,\theta}^{exp}} u(\theta, a, \omega)$. Therefore Algorithm \ref{alg:public_main} gets reward $OPT$ except rounds in first $|\A|\cdot |\varTheta|$ global phases. By Lemma \ref{lem:epoch}, we know that the expected number of rounds of the first  $|\A|\cdot |\varTheta|$ global phases is at most $C$. Therefore, Algorithm \ref{alg:public_main} has expected total reward at least  $\left(T - C \right) \cdot \OPT$.

\end{proof} 

==> stuff.tex <==
now for a very cool intro by alex slivkins!!
